Elephant in the Room: Dissecting and Reflecting on the Evolution of Online Social Network Research

Billions of individuals engage with Online Social Networks (OSN) daily. The owners of OSN try to meet the demands of their end-users while complying with business necessities. Such necessities may, however, lead to the adoption of restrictive data access policies that hinder research activities from "external" scientists -- who may, in turn, resort to other means (e.g., rely on static datasets) for their studies. Given the abundance of literature on OSN, we -- as academics -- should take a step back and reflect on what we have done so far, after having written thousands of papers on OSN. This is the first paper that provides a holistic outlook to the entire body of research that focused on OSN -- since the seminal work by Acquisti and Gross (2006). First, we search through over 1 million peer-reviewed publications, and derive 13,842 papers that focus on OSN: we organize the metadata of these works in the Minerva-OSN dataset, the first of its kind -- which we publicly release. Next, by analyzing Minerva-OSN, we provide factual evidence elucidating trends and aspects that deserve to be brought to light, such as the predominant focus on Twitter or the difficulty in obtaining OSN data. Finally, as a constructive step to guide future research, we carry out an expert survey (n=50) with established scientists in this field, and coalesce suggestions to improve the status quo such as an increased involvement of OSN owners. Our findings should inspire a reflection to "rescue" research on OSN. Doing so would improve the overall OSN ecosystem, benefiting both their owners and end-users and, hence, our society.

==> sections/archived/2-data-old.tex <==
\section{The Minerva-OSN Dataset}\label{sec:dataset}

Among our major contributions, we introduce the \dataset~dataset,\footnote{Minerva was the goddess of wisdom in Roman mythology.} used as basis to carry out our analysis and which we publicly release to downstream research. Let us elucidate the methodology -- which follows the guidelines of systematic analyses~\citep{booth2021systematic} -- employed in the construction of the \dataset~dataset.

\textbf{Venue selection.} We designed \dataset\ with the intention of collecting ``all'' OSN-related and \textit{peer-reviewed} papers that have ever been published. Hence, the first step entailed identifying the venues (i.e., journals and conference proceedings) that would contain such publications. We began our search with Google Scholar (among the most well-known repositories of scientific articles), analyzing the subcategories included in the ``Engineering and Science'' category: each subcategory lists the 20 most popular venues related to the subcategory. %\footnote{We selected all venues from the following subcategories: artificial intelligence, computational linguistics, computer security and cryptography, computer vision and pattern recognition, data mining and analyses, databases and information systems, human-computer interaction, and multimedia.} 
We integrated this list (we provide the full list in our repository) with all the venues included in Springer's Lecture Notes in Computer Science as well as the Association of Computing Machinery International Conference Proceedings Series. We manually reviewed all our identified venues, removing duplicates and merging venues that changed publisher or name (e.g., WWW becoming TheWebConf). Overall, we found 135 relevant venues. %(some of which are not ``active'' anymore, such as {\color{red}\textbf{XXX}}).

\textbf{Paper collection.} For each venue, we queried the Scopus database for \textit{all} papers that appeared therein---starting from 2006 (the year in which Facebook was released to the general public). For every paper, we collected its metadata; and specifically: title, authors (and affiliations), abstract, publication date, DOI. This led to over 1 million articles.

\textbf{Filtering papers on OSN.} There is no straightforward way to determine if any given paper is related to OSN. We hence designed a sensible heuristic: for each paper (among our 1+ million), we analyzed its abstract looking for \textit{mentions of the name of at least one OSN} (intuitively, a paper on OSN ``should'' mention an OSN in its abstract).\footnote{\textbf{Limitations.} Of course, we cannot claim that \dataset\ contains \textit{all} publications on OSN. Some papers may not be indexed in Scopus. Moreover, our selection of venues, despite its comprehensiveness, may have omitted some journals or conferences. Finally, our heuristic may have not captured papers that did not mention any specific OSN in the abstract.} To devise a list of OSN, we followed the procedure by \citet{fiesler2020no}, and relied on the Wikipedia page on OSN~\ref{link:wikipedia-osn-list}. For fairness, we considered the OSNs that were included in such web page for each year (e.g., the page is constantly updated, and some OSNs may be added or removed). Overall, we identified 280 unique OSN, which we used to carry out our search. To remove false positives, we further distill our results by (i) removing all papers that were published before the rollout of the ``matching'' OSN; and (ii) manually checking the results by looking for ``homonyms'', i.e., words that can be either used to denote an OSN or a completely different concept (e.g., ``bands''). 

\textbox{\textsc{\textbf{\dataset}.} After removing duplicates, we obtained 12,186 papers published in 2006--2023, spread among 135 venues, and which discuss one among 280 OSN (venues and OSN are listed in the Appendix). Our \dataset\ is the largest curated dataset of this kind that is specific to OSN research (and adheres to FAIR principles~\ref{fair}).}





\textbf{Paper collection.} For each venue, we queried the Scopus database for \textit{all} papers that appeared therein---starting from 2006 (the year in which Facebook was released to the general public). For every paper, we collected its metadata, i.e. title, authors (and affiliations), abstract, publication date, DOI. In total, we extracted over 1 million articles.

\textbf{Filtering papers on OSN.} There is no straightforward way to determine if any given paper is related to OSN. Hence, we designed a sensible \textit{heuristic}, which we applied to the abstract of every paper: 

\begin{enumerate}
    \item We examine each abstract for mentions of at least one OSN (intuitively, a paper on OSN ``should'' mention an OSN in its abstract).
    \item 
\end{enumerate}




The filtering process previously described requires a list of OSN. To devise a list of OSN, we followed the procedure by \citet{fiesler2020no}, and relied on the Wikipedia page on OSN~\ref{link:wikipedia-osn-list}. 
Furthermore, we enlarged this list with the integration alt-tech OSN~\ref{link:wikipedia-alttech-osn-list} and YouTube, a well-studied OSN in the literature that is not included in such lists~\cite{cheng2008statistics}. 
Overall, we identified 297 unique OSN, which we used to carry out our search.
Last, for each OSN, we identify a list of possible synonyms that can be used by researchers. 
The list is manually created:  for each OSN in our list, we search in Google Scholar scientific articles mentioning it (or in similar forms), and in Google the OSN history to spot potential changes in its name. 
For instance, researchers often call Weibo the OSN Shina Weibo, or, more generally, OSN whose name is composed of multiple names might be written differently (e.g., FilmAffinity is often called Filmaffinity). 

\textbf{Errors reduction techniques.}
To remove false positives, we further distill our results in various ways. First, by removing all papers that were published before the rollout of the ``matching'' OSN. 
Second, we restrict the research for OSN names that might have ``homonyms'', i.e., words that can be either used to denote an OSN or a completely different concept (e.g., ``bands''). 
For these, we maintain those research articles that contain at least one OSN mention and a list of keywords that can be linked to OSN, such as ``social network'', ``social platform'' etc. 
Third, the resulting database is manually inspected: for each OSN, we inspect up to 50 papers mentioning it.
Here, we remove articles that might mention a name belonging to OSN but that they not actually talk about OSN. 
In total, we removed 74 false positives. 
Interestingly, all false positives (except 1) belonged to unpopular OSN (OSN with less than 50 papers contained in our database). 
Finally, with this procedure, we created a dataset containing 13842 scientific articles discussing OSN. 
